Two-dimensional electrochemical model for mixed conductors: a study of ceria

A two-dimensional small bias model has been developed for a patterned metal current collector $|$ mixed oxygen ion and electronic conductor (MIEC) $|$ patterned metal current collector electrochemical cell in a symmetric gas environment. Specifically, we compute the electrochemical potential distributions of oxygen vacancies and electrons in the bulk and near the surface for $\text{Pt} | \text{Sm}_{0.15}\text{Ce}_{0.85}\text{O}_{1.925} | \text{Pt}$ symmetric cell in a $\text{H}_2-\text{H}_2\text{O}-\text{Ar}$ (reducing) atmosphere from 500 to $650^o C$. Using a two-dimensional finite-element model, we show that two types of electronic current exist within the cell: an in-plane drift-diffusion current that flows between the gas $|$ ceria chemical reaction site and the metal current collector, and a cross-plane current that flows between the two metal electrodes on the opposite side of the cell. By fitting the surface reaction constant $\tilde k_f^0$ to experimental electrode resistance values while fixing material properties such as bulk ionic and electronic equilibrium defect concentrations and mobilities, we are able to separate the electrode polarization into the surface reaction component and the in-plane electron drift-diffusion component. We show that for mixed conductors with a low electronic conductivity (a function of oxygen partial pressure) or a high surface reaction rate constant, the in-plane electron drift-diffusion resistance can become rate-limiting in the electrode reaction.

==> inputs/citations.tex <==
\cite{Adler-96}
\cite{Adler-97}
\cite{Kroger-56}
\cite{Polarons-62}
\cite{Liu-97}
\cite{Riess-86}
\cite{Riess-03}
\cite{Tschope-01}
\cite{Tschope-05}
\cite{Tschope-04}
\cite{Tuller-79}
\cite{Mogensen-00}
\cite{Sze-81}
\cite{Selberherr-84}
\cite{Rhoderick-00}
\cite{Fleig-05}
\cite{ISI:000258187300010}
\cite{ISI:000247314000018}
\cite{ISI:000242555200007}
\cite{ISI:000228521200050}
\cite{ISI:000226236100103}
\cite{ISI:000259269100064}
\cite{ISI:000252830600012}
\cite{ISI:000232773100001}
\cite{ISI:000227550500001}
\cite{ISI:A1975V426800018}
\cite{ISI:000168035300017}
\cite{ISI:000181439500003}
\cite{ISI:000178030100061}
\cite{ISI:A1973P856100037}



==> inputs/equilibrium_conditions.tex <==
We indicate the equilibrium conditions with superscript $(0)$. In order to determine equilibrium concentrations of vacancies and electrons, we consider the following defect reactions:
\begin{equation}
\begin{array}{lcl}
H_2({\rm gas})+O_2({\rm gas}) &\rightleftharpoons& H_2O({\rm gas}) \\
O_O^x  &\rightleftharpoons&V_O^{\bullet\bullet}+\frac{1}{2}O_2({\rm gas})+2e' 
\end{array}
\label{global_{eon}quilibrium_reactions}
\end{equation}
and the following equilibrium constants:
\begin{subequations}
\begin{eqnarray}
K_g = \displaystyle\frac{\tilde p_{H_2O}^2}{\tilde p_{H_2}^2\tilde p_{O_2}} \label{eqn:Kg}\\
K_r =  \displaystyle\left(\frac{c_{eon}^{(0)}}{B}\right)^2 \frac{c_{ion}^{(0)}}{B} \tilde p_{O_2}^{1/2}\\
1+ \displaystyle \frac{c_{eon}^{(0)}}{B} - 2\frac{c_{ion}^{(0)}}{B}=0
\end{eqnarray}
\label{eqns_global_reactions}
\end{subequations}
where  $\tilde p_k =\displaystyle \frac{p_k}{1 {\rm atm}}$ and $p_k$ is the partial pressure of species $k$. We solve the equilibrium concentrations of 
vacancies $c_{ion}^{(0)}$ and electrons $c_{eon}^{(0)}$ in the dilute limit at a given temperature and partial pressures.


%For SDC-15 we will have that the concentration of samaria atoms in the lattice $\left[ Sm_{Ce}' \right]=0.15 $, \cite{Kroger-56}, the $n_c$ coordination number is 4 \cite{Andersson03072006} and the cell length is $5.43\times 10^{-10}m$ \cite{zhan:A427} so its volume $V_0$ is given by $V_0 = l_{cell}^ 3$ this implies that the concentration of background negatively charged ions in the bulk can be expressed as $B = n_c \frac{\left[Sm_{Ce}'\right]}{V_0} = 3.74759\times10^{27}$.



==> inputs/input_data.tex <==
Input data is in Table \ref{table:diffusivity} and $W_1 = 1.5 \mu m$, $W_2 = 3\mu m$ and below

==> inputs/modeling_ceria.tex <==
Cerium oxides such as SDC exhibit mixed conducting behavior in reducing conditions. When SDC is subject to a electric potential excitation and to a chemical gradient it exhibits conductivity of oxygen ions and electrons. Oxygen ions motion is better understood as vacancy hopping, i.e. the hopping of vacant oxygen sites in the Ceria lattice, while electron conduction happens through thermally activated small polaron hopping (ref Tuller).  This complex behavior of  at the lattice scale can be averaged out at the mesoscale ($5 nm$ and up), and for electrons and vacancies we can write the following conservation equation ($m$ below can be $eon$, electron, or $ion$ for vacancies):
\begin{equation}
{\partial{c_m}\over{\partial t}}+\nabla\cdot \mathbf j_m^P=\dot{\Omega}_m
\label{eqn:charge_carrier_transport}
\end{equation}
where $c_m$ is the concentration of species $m$ expressed in terms of number of particles per unit volume $ \mathbf j_m^P$ is the particles $m$ flux and $\dot{\Omega}_m$ is the net rate of generation of the species $m$, typically taken to be zero in Ceria \cite{Tschope-01}.

The description of the charge transport in solids goes hand in hand with the description of the electo-magnetic fields arising in it. Magnetization effects are negligible and the dieletric field is assumed to be proportional to the electric field (ref. Applied physics paper I like with the dielectrics ), where the proportionality constant, the permittivity $\varepsilon$, varies little across the sample. According to these assumptions we can write that:
\begin{equation}
\nabla \cdot \left(\nabla \phi\right) =  -\frac{\rho}{\varepsilon}
\label{eqn:Poisson_phi}
\end{equation}
where $\rho$ is the background charge and $-\rho = e\left(B-\sum z_m c_m \right)= e\left(B+c_{eon}-2c_{ion}\right)$, where $z_m$ is an integer representing the charge of species m ($-1$ for electrons and $+2$ for vacancies)
We will indicate the operator $\nabla \cdot\left(\nabla (\cdot)\right)$ with the symbol $\triangle$.
The solutions of equations~\ref{eqn:charge_carrier_transport} and \ref{eqn:Poisson_phi} along with constitutive relations for the terms $\mathbf j_m^P = g_m\left(c_m, \nabla c_m, \nabla \phi, T, p\right)$, and appropriate boundary conditions will lead to the determination of the $c_m$'s and the $\phi$.
From non equilibrium thermodynamics, \cite{Prigogine-61} we can deduce that:
\begin{equation}
\mathbf j_m^P = -D_m c_m \nabla \frac{\tilde \mu_e}{k_bT} 
\end{equation}
where the electrochemical potential of species $m$ is given by: 
\begin{equation}
\tilde \mu_m = \mu^0_m + k_b T \log\left(\frac{c_m}{c_m^0} f_m(c_m, T,P)\right) + z_m e \phi
\label{eqn:electrochem_pot}
\end{equation}
where $\mu^0_m$ is the reference potential, $f_m(c_m, T, P)$ the activity coefficient dependent upon species concentration $c_m$, temperature $T$ and pressure $P$. We shall suppose in the reminder that $\nabla T = \nabla p =0$,  this is a good assumption given the system we simulate. Furthermore we suppose $f_m=1$ consistently with much of the literature, i.e. \cite{Adler-96}, \cite{Adler-97}, \cite{Liu-97}, \cite{Liu-99} and \cite{Riess-03}.
The \label{eqn:Poisson_phi}, \label{eqn:charge_carrier_transport} can be then rewritten in so-called self-consistent form as:
\begin{eqnarray}
\triangle \phi = \frac{e}{\varepsilon}\left( B+c_{eon}- 2c_{ion}\right)\\
\partial_t c_{eon}+\nabla\cdot\left(-D_{eon}\nabla c_{eon}+\frac{D_{eon}}{U_T} c_{eon}\nabla \phi\right)\\
\partial_t c_{ion}+\nabla\cdot\left(-D_{ion}\nabla c_{ion}-\frac{D_{ion}}{U_T} c_{ion}\nabla \phi\right)
\end{eqnarray}
We will refer the study of appropriate boundary conditions to the work of \cite{Adler-97}, \cite{Riess-07}



==> inputs/non_dimensional.tex <==
The solution of Equations (\ref{PDE_to_solve}) and (\ref{BC_to_solve}) gives $(n^{(1)}, \tilde \phi^{(1)})$ parametrized with respect to $\displaystyle \left(\frac{c_{ion}^{(0)}}{c_{eon}^{(0)}} \right.$, $\tilde A_\phi$, $\tilde A_n$, $W_1$, $W_2$, $\displaystyle \left.\frac{l_2}{l_c}\right)$ or, equivalently, to $\displaystyle\left(\frac{\tilde k_f \tilde p_{H_2}}{c_{ion}^{(0)}}\right.$, $\displaystyle\frac{D_{ion}}{D_{eon}}$, $\displaystyle\frac{c_{ion}^{(0)}}{c_{eon}^{(0)}}$, $W_1$, $\displaystyle\frac{W_2}{W_1}$, $\displaystyle\left.\frac{l_2}{l_c}\right)$. Since our focus is on SDC-15, the parameters $\displaystyle\frac{D_{ion}}{D_{eon}}$, $\displaystyle\frac{c_{ion}^{(0)}}{c_{eon}^{(0)}}$ are known well (refs), we also set the value of $\displaystyle\frac{l_2}{l_c}$ to be large and we remark that its value will not make much difference with respect to $R_{ion}^\perp$ if the Ceria sample is thick. On the other hand $\tilde k_f^0$, $W_1$, $\frac{W_2}{W_1}$ are not well known.

The previous comments summarize in the following way:
\begin{eqnarray}
\tilde \phi^{(1)} = f\left(\tilde x, \tilde y, \frac{\tilde k_f \tilde p_{H_2}}{c_{ion}^{(0)}}, W_1, \frac{W_1}{W_2}\right) \\
n^{(1)} = g\left(\tilde x, \tilde y, \frac{\tilde k_f \tilde p_{H_2}}{c_{ion}^{(0)}}, W_1, \frac{W_1}{W_2}\right)
\end{eqnarray}

Knowledge of $n^{(1)}$ and $\tilde \phi^{(1)}$ is interesting but appropriate integrals of $n^{(1)}$ and $\phi^{(1)}$ are more interesting because the directly relate to measurable quantities.
%In particular we shall note that:
%\begin{eqnarray}
%\displaystyle  R_{ion}^\perp = \frac{<\tilde \mu_{eon}^\star>_{\Gamma_4}-<\tilde \mu_{ion}^\star>_{\Gamma_5}}{j_g}\\
%\displaystyle R_{pol} =   \frac{<\tilde \mu_{eon}^\star>_{\varphi_e^S(\Gamma_5)}-< \tilde\mu_{ion}^\star>_{\Gamma_5}}{j_g}\\
%\displaystyle R_{surf} =  \left( 1+\frac{\bar n}{4 \bar p}\right)\frac{<n^{(1)}>_{\Gamma_5}}{j_g}
%\end{eqnarray}
We note that:
\begin{equation}
j_g =\frac{1}{(W_1+W_2)}D_{eon} e c_{eon}^{(0)}\int_{\Gamma_5}\partial_{\tilde y}\left( \tilde\phi^{1}- \partial_{\tilde y}  n^{(1)} \right)\ud \tilde x
\end{equation}
thus:
\begin{eqnarray}
\displaystyle  R_{ion}^\perp = \frac{W_1+W_2}{W_2} \frac{1}{D_{eon} e c_{eon}^{(0)}} \frac{<\tilde \mu_{eon}^\star>_{\Gamma_4}-<\tilde \mu_{ion}^\star>_{\Gamma_5}}{<\partial_{\tilde y} \tilde\phi^{1}- \partial_{\tilde y}  n^{(1)} >_{\Gamma_5}}\\
\displaystyle R_{pol} = \frac{W_1+W_2}{W_2} \frac{1}{D_{eon} e c_{eon}^{(0)}}  \frac{<\tilde \mu_{eon}^\star>_{\varphi_e^S(\Gamma_5)}-< \tilde\mu_{ion}^\star>_{\Gamma_5}}{<\partial_{\tilde y} \tilde\phi^{1}- \partial_{\tilde y}  n^{(1)} >_{\Gamma_5}}\\
\displaystyle R_{surf} =  \frac{W_1+W_2}{W_2} \frac{1}{D_{eon} e c_{eon}^{(0)}}  \left( 1+\frac{\bar n}{4 \bar p}\right)\frac{<n^{(1)}>_{\Gamma_5}}{<\partial_{\tilde y} \tilde\phi^{1}- \partial_{\tilde y}  n^{(1)} >_{\Gamma_5}}
\end{eqnarray}

So we can derive $R_{ion}^\perp$, $R_{pol}$ and $R_{surf}$ depend semi-linearly upon $\frac{W_1+W_2}{W_2} \frac{1}{D_{eon} e c_{eon}^{(0)}}$. Their ratios will be then:

\begin{eqnarray}
\displaystyle f_{eon-DD} = \frac{<\tilde \mu_{eon}^\star>_{\varphi_e^S(\Gamma_5)}-< \tilde\mu_{ion}^\star>_{\Gamma_5}}{<\tilde \mu_{eon}^\star>_{\Gamma_4}-<\tilde \mu_{ion}^\star>_{\Gamma_5}}\\
\displaystyle f_{surf} =  \left( 1+\frac{\bar n}{4 \bar p}\right)\frac{<n^{(1)}>_{\Gamma_5}}{<\tilde \mu_{eon}^\star>_{\Gamma_4}-<\tilde \mu_{ion}^\star>_{\Gamma_5}}\end{eqnarray}



==> inputs/topological_considerations.tex <==
We define  $\varphi_e$ the flow generated by the vector field $\mathbf j_e$. It is interesting to study how $\Gamma_5$ transforms under $\varphi_e$: if we take a current line departing from the Gas-Ceria interface we are interested to know where it ends up. A currently physically describes some averaged motion of the electrons which flow in the bulk. This "motion" describes an influence region for the chemical electrons both in the bulk and metal phases. We indicate these regions are $\varphi_e(\Gamma_5)$ and $\varphi_e(\Gamma_5)\cap \Gamma_4=:\varphi^S(\Gamma_5)$. We note that obviously this influence region is not $\Omega$ but a small subset of it restricted to the vicinity of $\Gamma_5$. Its schematic depiction is given in Fig.~\ref{fig:Topology}
. Parameters can can be used to describe it are it area $A$, the length of its outer line $l_{max}$, the penetration depth $d_{max}$ and the fraction of the region affected by the $\max(m(\varphi_e(\Gamma_5)\cap \Gamma_4 ))/m(\Gamma_4)$.
